A Checklist for the Evaluation of Pedestrian Simulation Software Functionalities

The employment of micro-simulation (agent-based) tools in the phase of design of public and private spaces and facilities and for the definition of transport schemes that impact on pedestrian flows, thanks to their achieved accuracy and predictive capacity, has become a consolidated practice. These instruments provide support to the organization of spaces, services and facilities and to the definition of management procedures for normal and emergency situations. The employment of these tools is effective for various but not for all the contexts, nevertheless new features and functions are under constant development and new products are often launched on the market. Therefore, there is a higher necessity of a standard criteria both for the evaluation of the kinds of function that these software provide, at use of practitioners and end-users, and for the definition of software requirements as a reference for the developers that aim at being competitive on this market. On the basis of our experience as pedestrian modellers and as researchers in the crowd modelling area, we designed a comprehensive and detailed ready-to-use checklist for the quantitative evaluation of Pedestrian Simulation Software functionalities that aims at capturing all the aspects that we claim that are useful to undertake a professional study. These functions in our opinion are necessary to provide accurate results in the planning of new facilities or schemes that involve pedestrian activities. With this work we propose a set of criteria of evaluation for these products also to encourage a debate for the definition of objective standards for pedestrian simulation software certification.

==> ArXvi_intro_Sara.tex <==

\begin{abstract}

The employment of micro-simulation (agent-based) tools in the phase of design of public and private spaces and facilities and for the definition of transport schemes that impact on pedestrian flows, thanks to their achieved accuracy and predictive capacity, has become a consolidated practice. These instruments provide support to the organization of spaces, services and facilities and to the definition of management procedures for normal and emergency situations. The employment of these tools is effective for various but not for all the contexts, nevertheless new features and functions are under constant development and new products are often launched on the market. Therefore, there is a higher necessity of a standard criteria both for the evaluation of the kinds of function that these software provide, at use of practitioners and end-users, and for the definition of software requirements as a reference for the developers that aim at being competitive on this market.

On the basis of our experience as pedestrian modellers and as researchers in the crowd modelling area, we designed a comprehensive and detailed ready-to-use checklist for the quantitative evaluation of Pedestrian Simulation Software functionalities that aims at capturing all the aspects that we claim that are useful to undertake a professional study. These functions in our opinion are necessary to provide accurate results in the planning of new facilities or schemes that involve pedestrian activities. With this work we propose a set of criteria of evaluation for these products also to encourage a debate for the definition of objective standards for pedestrian simulation software certification.
\end{abstract}

\keywords pedestrian simulation, agent-base models, evaluation, crowd simulation

\section{Introduction}

Simulation studies of crowds and pedestrian dynamics are nowadays more and more required in the phases of assessment and design of public and private spaces and facilities and they constitute valid tools for the support of the work of Architects, Engineers, Urban Planners, Decision makers, Security managers and so on. The use of simulation instruments successfully shows advantages in heterogeneous contexts such as transit stations (underground, railway, bus terminal), airports, sport venues (stadium, arenas, urban sport events), retails (shopping centers, supermarkets), private and public buildings (schools, prisons), entertainment (theaters, cinemas, concerts) and large events. Micro-Simulation tools have therefore become sufficiently reliable to predict with accuracy, in specific contexts of application (and if informed with a reliable demand), the characteristics of pedestrian dynamics and flows and to highlight in advance possible criticalities. They also allow to: dimension the number of pedestrian facilities or operative components, like gates or Vertical Circulation Elements (VCE) for normal and emergency operations; predict egress and evacuation times; assess the performance of different functional areas of the environment; evaluate operative procedures; compare the efficiency of different layouts or configurations of the environment; study worst-case/what-if scenarios and disruptions that are not directly observable in reality; support the definition of strategies of crowd management and decision making; optimize the positioning of specific services and of sign-posting; assess the accessibility and movement of People with Restricted Mobility (PRMs); perform social cost analysis etc. 

% Some of these software also allow to import Fire Dynamic Simulation (FDS) data for evacuation scenarios. Smoke and Fire simulation data are imported from platforms like SmartFire\footnote{University of Greenwich, \url{http://fseg.gre.ac.uk/smartfire/}} or other Computational Fluid Dynamics simulation software that allow to simulate the propagation of fire, smoke, thermal radiation and toxicity in indoor environments, provided the volume of the environment and the kind of materials present in the scenario. 

%\begin{table}[!h]
	%\caption{List of most diffused pedestrian simulation platforms}
	%\label{tab:software}
%\begin{center}
%\scriptsize
	%\begin{tabular}{|l|l|l|}
%\hline
%Name & Developer  & Website \\
%\hline \hline
%SpaceWorks & Legion ltd & \url{http://www.legion.com/legion-spaceworks/}\\
%\hline
%VisWalk & PTV AG & \url{http://vision-traffic.ptvgroup.com/}\\
%\hline
%STEPS & Mott MacDonald Group ltd & \url{http://www.steps.mottmac.com/} \\
%\hline
%MassMotion & Oasys ltd & \url{http://www.oasys-software.com/}\\
%\hline
%Paramics & Pitney Bowes Business & \url{http://www.paramics-online.com/}\\
%\hline
%CAST Pedestrian & Airport Research Center GmbH &  \url{http://www.airport-consultants.com} \\
%\hline
%%CAST Terminal & Airport Research Center GmbH &  \url{http://www.airport-consultants.com} \\
%%\hline
%PedGo & TraffGo HT GmbH & \url{http://traffgo-ht.com/} \\
%\hline
%SimWalk & Savannah Simulations AG & \url{http://www.simwalk.com/}\\
%\hline
%Event Planner & Crowd Dynamics ltd & \url{http://www.crowddynamics.com/}\\
%\hline
%Exodus & University of Greenwich & \url{http://fseg.gre.ac.uk/exodus/}\\
%\hline
%\end{tabular}
%\end{center}
%\end{table}


The scheme in Fig. \ref{fig:flusso} shows the typical workflow of the simulation process. The first step is the information of the model. The great part of these platforms allows to import the layout of the environment in a CAD drawing form and to import Origin-Destination matrices (OD matrices) of pedestrian flows combined with an event schedule. These data inform the model with the observed or predicted demand. The demand is usually prepared on the basis of a data collection campaign performed onsite (i.e. people headcounts in a station). If the simulated environment does not exist yet, simulation tools can still be used in the design process for the comparison of predicted performances of alternative options (layout, services, demand etc.). In this case the demand has to be shaped by techniques of demand forecasting.

Then, in the phase of dynamic modelling, the base model has to be calibrated and validated. Only then variations of the base model (i.e. what-if scenarios that might include alternative design, time schedule variations or evacuation scenarios) can be considered reliable. 

In the phase of analysis, simulation analysis tools allow extracting quantitative and qualitative data from simulation runs. Pedestrian  dynamics can be visualized in 2D or 3D and outputs can be extracted in a numerical form or analyzed in the form of charts or maps of various kinds. Data that can usually be extracted from these software are related to density, occupancy times, transfer times, delays and so on.

\begin{figure}[h]
	\centering
	\includegraphics[width=\columnwidth]{flusso.png}
	\caption{The simulation process}
	\label{fig:flusso}
\end{figure}

%MODIFICHE SARA DA QUI

The visualization of pedestrian and mobility dynamics provided by some pedestrian simulation software can be extremely advanced but it is clear that, the accuracy of the reproduced dynamics, and the consequent performance prediction, relies on the accurate information of the simulation model, on the precise reproduction of the layout under study, and on a proper calibration and validation of the model.


%On the basis of our experience as users (in terms of pedestrian modelers) of commercial platforms and as researchers in the crowd modelling area, we designed a \emph{detailed checklist for the evaluation of Pedestrian Simulation Software} that aims at capturing all the required aspects to undertake a professional study and, therefore, to provide accurate results in the planning of new facilities or transport schemes that have impact on pedestrian flow. With this work we propose a set of criteria of evaluation for these products that also aims at starting a debate for the definition of objective standards for pedestrian simulation software certification.

In this paper we present a \emph{detailed checklist for the evaluation of Pedestrian Simulation Software} that we designed with reference to our experience both as users of commercial platforms for pedestrian dynamics, and as researchers in the crowd modelling area and agent-based approach for tackling complex systems. We believe that the ready-to-use and intuitive checklist that we propose here might be perceived as a first draft of standard criteria for the evaluation of pedestrian simulation software. We claim that the potential value of this checklist is twofold: for practitioners in modelling activity, as tool towards the selection of the most appropriate platform for their needs, and also for developers of pedestrian dynamics software to drive their choices in the improvement of their products.

%In particular the proposed checklist would be useful to evaluate the completeness of a proposed software against a comprehensive list of possible functions. These functions have been determined on the basis of what we perceive, under the practitioner's point of view, as the tools that are fundamental to undertake an accurate pedestrian modelling study.
%In other words, this checklist would help to quickly check if a function is provided or not by a software, at the modelling, analysis and presentation's level. 

%For example it would help to determine if advanced and complex dynamics can be modelled, also with the help of logical conditions, or if all kinds of Vertical Circulation Elements can be represented in the simulation environment and so on. On the analysis level it would help to understand what kind of data can be extracted from the software and if advanced and customized analysis can be performed.

At our knowledge general evaluation criteria for pedestrian simulation software do not exist. In spite the availability of several software products, in fact, they hardly refer to the same functional and technical requirements and, thus, their comparison is difficult and usually based on the experimentation of a couple of them on given scenarios (see e.g. \cite{castle2011comparison}, \cite{xiao2005methodology}, \cite{haron2012software}).

Differently, we started from modelling and analysis functionalities we judged mandatory for professional modelling activities (without reference to any specific scenario or software) to built up the checklist presented in the following. In our opinion, a lack of expressive capacity for representing the environment, pedestrian dynamics or scheduled events and poor analysis functionalities, inevitably ends up in an over approximation of reality under study with consequent limited accuracy and quality of the study itself. Although we have applied our criteria of evaluation to a few software and we found it useful and effective, here we will not refer to any specific software.

In the design of the checklist we moreover took into account previous developed comparisons and international references available in the international literature, e.g. about high-level user-oriented guidelines for the choice of evacuation models/software \cite{kuligowski2005user} and key questions a final user should answer proposed in\cite{castle2007guidelines}, but also available comparisons of given softwares like in \cite{AlexanderssonJohansson:Thesis2013}.


%Our intention is therefore to propose a common ground for software comparison. Although what we propose is a quantitative checklist that summarizes the functions that a pedestrian simulation software might have, without offering a method to judge also qualitatively each specific function, we believe that the quality of the studies undertaken with these tools is definitely highly dependent on the modelling and analysis options made available in each software, in addition to the modeller's skills. A lack of expressive capacity for the definition of the environment, pedestrian dynamics or scheduled events and poor analysis possibilities, in our opinion, inevitably ends up in an excessive approximation of reality, in the simulation, that would reflect also on the accuracy and quality of the final results of the study.

%At our knowledge it does not exist a general evaluation criteria of these platforms that reflects the simulation process performed according to the simulation best practices (see \cite{nikoukaran1998criteria} for a more general work on the evaluation of simulation software). 

%Although we have applied our criteria of evaluation to a few software and we found it useful and effective, here we will not refer to any specific software, differently from works like \cite{castle2011comparison} \cite{xiao2005methodology} \cite{haron2012software} that compare the use of specific competitor platforms on the same scenario. 

%Some high-level user-oriented guidelines for the choice of evacuation models/software can be also found in \cite{kuligowski2005user}. In \cite{castle2007guidelines} the author instead proposes some key questions a final user should answer to choose accurately an evacuation software after introducing in details different formal models that the platforms can embedded. See also \cite{AlexanderssonJohansson:Thesis2013} for similar criteria of comparison declined on two specific software.

The remaining of the paper is organized as follows: Section 2 will give an high-level overview of the aspects that we believe are important for the evaluation of the characteristics and functionalities of a pedestrian simulation software; Section 3 will list in details, for each of the considered aspects, the specific functionalities that are relevant from our viewpoint together with a description accessible also to not experts final users; Section 4 will describe the proposed quantitative criteria we suggest for software evaluation; paper ends with final remarks and future works in Section 5.

\section{Requirements: High-level Categorization}
\label{sec:overview}

In this Section we introduce in a form of high-level categorization organized in three subsets the features that we think should be supported by pedestrian simulation platforms. Every subset collects all the features which support specific aspects of the process of the definition of a pedestrian simulation. 		

\begin{figure}[!hb]
	\centering
	\includegraphics[width=\columnwidth]{overview.png}
	\caption{The scheme above summarizes the high-level categorization}
	\label{fig:overview}
\end{figure}

The three subsets are identified as follows (see Fig. \ref{fig:overview}):

\begin{enumerate}
\item SCENARIO (subset 1): functions supporting the definition of the simulated \emph{scenario}. In this subset we refer to all the aspects dedicated to the preparation of the scenario where the dynamic simulation will take place. The scenario definition implies the possibility of manipulation of the physical environment (e.g. by means of CAD files that can be imported and manipulated to obtain the basic environment of the simulation) (subset 1\emph{(a)}), the characterization of its operative elements (stairs, escalators, lifts, ticket windows and so on) and of the routing elements that would guide pedestrians through the environment and that would influence their decisions (subset 1\emph{(b)}). The scenario definition also includes the possibility to inform the model by means of OD-matrices and the possibility to vary the mode of the simulation (subset 1\emph{(c)});

\item PEDESTRIANS (subset 2): functions supporting the possibility to model different types of pedestrians by varying their physical characteristics as speed, size, encumbrance, and also their behavioral components such as decision making processes. Some advanced features might include the cohesion of a group, a partial \emph{a-priori} knowledge of the environment and the possibility to define emotional states;

\item OUTPUT (subset 3): functions supporting the extraction of simulation \emph{output} to perform analysis and to export and visualize data related to density, delay times, distances, pedestrian counting and so on. A set of tools for the management and the presentation of outputs in the form of maps and charts and that includes the possibility of performing some data filtering should be provided by the platform.
\end{enumerate}

In the next Section we describe each of the above listed subsets in details.



==> to submit - senza table e reference/ArXvi_intro_Sara.tex <==

\begin{abstract}

The employment of micro-simulation (agent-based) tools in the phase of design of public and private spaces and facilities and for the definition of transport schemes that impact on pedestrian flows, thanks to their achieved accuracy and predictive capacity, has become a consolidated practice. These instruments provide support to the organization of spaces, services and facilities and to the definition of management procedures for normal and emergency situations. The employment of these tools is effective for various but not for all the contexts, nevertheless new features and functions are under constant development and new products are often launched on the market. Therefore, there is a higher necessity of a standard criteria both for the evaluation of the kinds of function that these software provide, at use of practitioners and end-users, and for the definition of software requirements as a reference for the developers that aim at being competitive on this market.

On the basis of our experience as pedestrian modellers and as researchers in the crowd modelling area, we designed a comprehensive and detailed ready-to-use checklist for the quantitative evaluation of Pedestrian Simulation Software functionalities that aims at capturing all the aspects that we claim that are useful to undertake a professional study. These functions in our opinion are necessary to provide accurate results in the planning of new facilities or schemes that involve pedestrian activities. With this work we propose a set of criteria of evaluation for these products also to encourage a debate for the definition of objective standards for pedestrian simulation software certification.
\end{abstract}

\keywords pedestrian simulation, agent-base models, evaluation, crowd simulation

\section{Introduction}

Simulation studies of crowds and pedestrian dynamics are nowadays more and more required in the phases of assessment and design of public and private spaces and facilities and they constitute valid tools for the support of the work of Architects, Engineers, Urban Planners, Decision makers, Security managers and so on. The use of simulation instruments successfully shows advantages in heterogeneous contexts such as transit stations (underground, railway, bus terminal), airports, sport venues (stadium, arenas, urban sport events), retails (shopping centers, supermarkets), private and public buildings (schools, prisons), entertainment (theaters, cinemas, concerts) and large events. Micro-Simulation tools have therefore become sufficiently reliable to predict with accuracy, in specific contexts of application (and if informed with a reliable demand), the characteristics of pedestrian dynamics and flows and to highlight in advance possible criticalities. They also allow to: dimension the number of pedestrian facilities or operative components, like gates or Vertical Circulation Elements (VCE) for normal and emergency operations; predict egress and evacuation times; assess the performance of different functional areas of the environment; evaluate operative procedures; compare the efficiency of different layouts or configurations of the environment; study worst-case/what-if scenarios and disruptions that are not directly observable in reality; support the definition of strategies of crowd management and decision making; optimize the positioning of specific services and of sign-posting; assess the accessibility and movement of People with Restricted Mobility (PRMs); perform social cost analysis etc. 

% Some of these software also allow to import Fire Dynamic Simulation (FDS) data for evacuation scenarios. Smoke and Fire simulation data are imported from platforms like SmartFire\footnote{University of Greenwich, \url{http://fseg.gre.ac.uk/smartfire/}} or other Computational Fluid Dynamics simulation software that allow to simulate the propagation of fire, smoke, thermal radiation and toxicity in indoor environments, provided the volume of the environment and the kind of materials present in the scenario. 

%\begin{table}[!h]
	%\caption{List of most diffused pedestrian simulation platforms}
	%\label{tab:software}
%\begin{center}
%\scriptsize
	%\begin{tabular}{|l|l|l|}
%\hline
%Name & Developer  & Website \\
%\hline \hline
%SpaceWorks & Legion ltd & \url{http://www.legion.com/legion-spaceworks/}\\
%\hline
%VisWalk & PTV AG & \url{http://vision-traffic.ptvgroup.com/}\\
%\hline
%STEPS & Mott MacDonald Group ltd & \url{http://www.steps.mottmac.com/} \\
%\hline
%MassMotion & Oasys ltd & \url{http://www.oasys-software.com/}\\
%\hline
%Paramics & Pitney Bowes Business & \url{http://www.paramics-online.com/}\\
%\hline
%CAST Pedestrian & Airport Research Center GmbH &  \url{http://www.airport-consultants.com} \\
%\hline
%%CAST Terminal & Airport Research Center GmbH &  \url{http://www.airport-consultants.com} \\
%%\hline
%PedGo & TraffGo HT GmbH & \url{http://traffgo-ht.com/} \\
%\hline
%SimWalk & Savannah Simulations AG & \url{http://www.simwalk.com/}\\
%\hline
%Event Planner & Crowd Dynamics ltd & \url{http://www.crowddynamics.com/}\\
%\hline
%Exodus & University of Greenwich & \url{http://fseg.gre.ac.uk/exodus/}\\
%\hline
%\end{tabular}
%\end{center}
%\end{table}


The scheme in Fig. \ref{fig:flusso} shows the typical workflow of the simulation process. The first step is the information of the model. The great part of these platforms allows to import the layout of the environment in a CAD drawing form and to import Origin-Destination matrices (OD matrices) of pedestrian flows combined with an event schedule. These data inform the model with the observed or predicted demand. The demand is usually prepared on the basis of a data collection campaign performed onsite (i.e. people headcounts in a station). If the simulated environment does not exist yet, simulation tools can still be used in the design process for the comparison of predicted performances of alternative options (layout, services, demand etc.). In this case the demand has to be shaped by techniques of demand forecasting.

Then, in the phase of dynamic modelling, the base model has to be calibrated and validated. Only then variations of the base model (i.e. what-if scenarios that might include alternative design, time schedule variations or evacuation scenarios) can be considered reliable. 

In the phase of analysis, simulation analysis tools allow extracting quantitative and qualitative data from simulation runs. Pedestrian  dynamics can be visualized in 2D or 3D and outputs can be extracted in a numerical form or analyzed in the form of charts or maps of various kinds. Data that can usually be extracted from these software are related to density, occupancy times, transfer times, delays and so on.

\begin{figure}[h]
	\centering
	\includegraphics[width=\columnwidth]{flusso.png}
	\caption{The simulation process}
	\label{fig:flusso}
\end{figure}

%MODIFICHE SARA DA QUI

The visualization of pedestrian and mobility dynamics provided by some pedestrian simulation software can be extremely advanced but it is clear that, the accuracy of the reproduced dynamics, and the consequent performance prediction, relies on the accurate information of the simulation model, on the precise reproduction of the layout under study, and on a proper calibration and validation of the model.


%On the basis of our experience as users (in terms of pedestrian modelers) of commercial platforms and as researchers in the crowd modelling area, we designed a \emph{detailed checklist for the evaluation of Pedestrian Simulation Software} that aims at capturing all the required aspects to undertake a professional study and, therefore, to provide accurate results in the planning of new facilities or transport schemes that have impact on pedestrian flow. With this work we propose a set of criteria of evaluation for these products that also aims at starting a debate for the definition of objective standards for pedestrian simulation software certification.

In this paper we present a \emph{detailed checklist for the evaluation of Pedestrian Simulation Software} that we designed with reference to our experience both as users of commercial platforms for pedestrian dynamics, and as researchers in the crowd modelling area and agent-based approach for tackling complex systems. We believe that the ready-to-use and intuitive checklist that we propose here might be perceived as a first draft of standard criteria for the evaluation of pedestrian simulation software. We claim that the potential value of this checklist is twofold: for practitioners in modelling activity, as tool towards the selection of the most appropriate platform for their needs, and also for developers of pedestrian dynamics software to drive their choices in the improvement of their products.

%In particular the proposed checklist would be useful to evaluate the completeness of a proposed software against a comprehensive list of possible functions. These functions have been determined on the basis of what we perceive, under the practitioner's point of view, as the tools that are fundamental to undertake an accurate pedestrian modelling study.
%In other words, this checklist would help to quickly check if a function is provided or not by a software, at the modelling, analysis and presentation's level. 

%For example it would help to determine if advanced and complex dynamics can be modelled, also with the help of logical conditions, or if all kinds of Vertical Circulation Elements can be represented in the simulation environment and so on. On the analysis level it would help to understand what kind of data can be extracted from the software and if advanced and customized analysis can be performed.

At our knowledge general evaluation criteria for pedestrian simulation software do not exist. In spite the availability of several software products, in fact, they hardly refer to the same functional and technical requirements and, thus, their comparison is difficult and usually based on the experimentation of a couple of them on given scenarios (see e.g. \cite{castle2011comparison}, \cite{xiao2005methodology}, \cite{haron2012software}).

Differently, we started from modelling and analysis functionalities we judged mandatory for professional modelling activities (without reference to any specific scenario or software) to built up the checklist presented in the following. In our opinion, a lack of expressive capacity for representing the environment, pedestrian dynamics or scheduled events and poor analysis functionalities, inevitably ends up in an over approximation of reality under study with consequent limited accuracy and quality of the study itself. Although we have applied our criteria of evaluation to a few software and we found it useful and effective, here we will not refer to any specific software.

In the design of the checklist we moreover took into account previous developed comparisons and international references available in the international literature, e.g. about high-level user-oriented guidelines for the choice of evacuation models/software \cite{kuligowski2005user} and key questions a final user should answer proposed in\cite{castle2007guidelines}, but also available comparisons of given softwares like in \cite{AlexanderssonJohansson:Thesis2013}.


%Our intention is therefore to propose a common ground for software comparison. Although what we propose is a quantitative checklist that summarizes the functions that a pedestrian simulation software might have, without offering a method to judge also qualitatively each specific function, we believe that the quality of the studies undertaken with these tools is definitely highly dependent on the modelling and analysis options made available in each software, in addition to the modeller's skills. A lack of expressive capacity for the definition of the environment, pedestrian dynamics or scheduled events and poor analysis possibilities, in our opinion, inevitably ends up in an excessive approximation of reality, in the simulation, that would reflect also on the accuracy and quality of the final results of the study.

%At our knowledge it does not exist a general evaluation criteria of these platforms that reflects the simulation process performed according to the simulation best practices (see \cite{nikoukaran1998criteria} for a more general work on the evaluation of simulation software). 

%Although we have applied our criteria of evaluation to a few software and we found it useful and effective, here we will not refer to any specific software, differently from works like \cite{castle2011comparison} \cite{xiao2005methodology} \cite{haron2012software} that compare the use of specific competitor platforms on the same scenario. 

%Some high-level user-oriented guidelines for the choice of evacuation models/software can be also found in \cite{kuligowski2005user}. In \cite{castle2007guidelines} the author instead proposes some key questions a final user should answer to choose accurately an evacuation software after introducing in details different formal models that the platforms can embedded. See also \cite{AlexanderssonJohansson:Thesis2013} for similar criteria of comparison declined on two specific software.

The remaining of the paper is organized as follows: Section 2 will give an high-level overview of the aspects that we believe are important for the evaluation of the characteristics and functionalities of a pedestrian simulation software; Section 3 will list in details, for each of the considered aspects, the specific functionalities that are relevant from our viewpoint together with a description accessible also to not experts final users; Section 4 will describe the proposed quantitative criteria we suggest for software evaluation; paper ends with final remarks and future works in Section 5.

\section{Requirements: High-level Categorization}
\label{sec:overview}

In this Section we introduce in a form of high-level categorization organized in three subsets the features that we think should be supported by pedestrian simulation platforms. Every subset collects all the features which support specific aspects of the process of the definition of a pedestrian simulation. 		

\begin{figure}[!hb]
	\centering
	\includegraphics[width=\columnwidth]{overview.png}
	\caption{The scheme above summarizes the high-level categorization}
	\label{fig:overview}
\end{figure}

The three subsets are identified as follows (see Fig. \ref{fig:overview}):

\begin{enumerate}
\item SCENARIO (subset 1): functions supporting the definition of the simulated \emph{scenario}. In this subset we refer to all the aspects dedicated to the preparation of the scenario where the dynamic simulation will take place. The scenario definition implies the possibility of manipulation of the physical environment (e.g. by means of CAD files that can be imported and manipulated to obtain the basic environment of the simulation) (subset 1\emph{(a)}), the characterization of its operative elements (stairs, escalators, lifts, ticket windows and so on) and of the routing elements that would guide pedestrians through the environment and that would influence their decisions (subset 1\emph{(b)}). The scenario definition also includes the possibility to inform the model by means of OD-matrices and the possibility to vary the mode of the simulation (subset 1\emph{(c)});

\item PEDESTRIANS (subset 2): functions supporting the possibility to model different types of pedestrians by varying their physical characteristics as speed, size, encumbrance, and also their behavioral components such as decision making processes. Some advanced features might include the cohesion of a group, a partial \emph{a-priori} knowledge of the environment and the possibility to define emotional states;

\item OUTPUT (subset 3): functions supporting the extraction of simulation \emph{output} to perform analysis and to export and visualize data related to density, delay times, distances, pedestrian counting and so on. A set of tools for the management and the presentation of outputs in the form of maps and charts and that includes the possibility of performing some data filtering should be provided by the platform.
\end{enumerate}

In the next Section we describe each of the above listed subsets in details.


